Nearly Tight Bounds For Differentially Private Min $s$-$t$ and Multiway Cut

Finding min $s$-$t$ cuts in graphs is a basic algorithmic tool with applications in image segmentation, community detection, reinforcement learning, and data clustering. In this problem, we are given two nodes as terminals, and the goal is to remove the smallest number of edges from the graph so that these two terminals are disconnected. We study the complexity of differential privacy for the min $s$-$t$ cut problem and show nearly tight lower and upper bounds where we achieve privacy at no cost for running time efficiency. We also develop a differentially private algorithm for the multiway $k$-cut problem, in which we are given $k$ nodes as terminals that we would like to disconnect. As a function of $k$, we obtain privacy guarantees that are exponentially more efficient than applying the advanced composition theorem to known algorithms for multiway $k$-cut. Finally, we empirically evaluate the approximation of our differentially private min $s$-$t$ cut algorithm and show that it almost matches the quality of the output of non-private ones.

==> Future.tex <==
\section{Conclusion And Future Work}
In this work, we investigate the differential privacy of the min $s$-$t$ cut and of, its generalization, the multiway $k$-cut problem. For the first problem, we show almost tight lower- and upper-bounds in terms of the error guarantee. Moreover, our DP algorithm is as fast as the fastest non-private one. For the multiway $k$-cut problem, we develop a novel approach that yields only $O(n/\eps \cdot \log k)$ additive error, as opposed to $O(n /\eps \cdot k)$ that standard algorithms lead to, in order to achieve DP. This algorithm might be of independent interest.
In particular, the \emph{total} running time of our multiway $k$-cut algorithm is only $O(\log k)$ more than that of the fastest non-private min $s$-$t$ cut. This is in stark contrast with the prior non-private $2$-approximate approach, which is $O(k)$ times slower than the fastest non-private min $s$-$t$ cut algorithm.

Comparing our lower- and upper-bounds, it remains to close the gap of $1/\eps$ multiplicative factor in the additive error of the min $s$-$t$ cut problem. It also remains open whether $O(\log k)$ factor in the additive error for the multiway $k$-cut problem is needed. We believe that techniques relying on solving LPs might be able to avoid this dependence on $O(\log k)$.
Finally, it would be interesting to explore whether smaller additive error is possible for special but interesting classes of graphs.
